Nonlinear PCA for Spatio-Temporal Analysis of Earth Observation Data

Remote sensing observations, products and simulations are fundamental sources of information to monitor our planet and its climate variability. Uncovering the main modes of spatial and temporal variability in Earth data is essential to analyze and understand the underlying physical dynamics and processes driving the Earth System. Dimensionality reduction methods can work with spatio-temporal datasets and decompose the information efficiently. Principal Component Analysis (PCA), also known as Empirical Orthogonal Functions (EOF) in geophysics, has been traditionally used to analyze climatic data. However, when nonlinear feature relations are present, PCA/EOF fails. In this work, we propose a nonlinear PCA method to deal with spatio-temporal Earth System data. The proposed method, called Rotated Complex Kernel PCA (ROCK-PCA for short), works in reproducing kernel Hilbert spaces to account for nonlinear processes, operates in the complex kernel domain to account for both space and time features, and adds an extra rotation for improved flexibility. The result is an explicitly resolved spatio-temporal decomposition of the Earth data cube. The method is unsupervised and computationally very efficient.We illustrate its ability to uncover spatio-temporal patterns using synthetic experiments and real data. Results of the decomposition of three essential climate variables are shown: satellite-based global Gross Primary Productivity (GPP) and Soil Moisture (SM), and reanalysis Sea Surface Temperature (SST) data. The ROCK-PCA method allows identifying their annual and seasonal oscillations, as well as their non-seasonal trends and spatial variability patterns.

==> authorsBibliography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,keepaspectratio]{images/diego.png}}]%
{Diego Bueso}
obtained his degree in Physics (2016), a Master degree in Remote sensing (2017) from the Universitat de Val\`encia. He is currently a Ph.D. degree at the Image and Signal Processing (ISP) working on machine learning applications on geoscience.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/maria.png}}]{Maria Piles} (S’05–M’11) received the M.S. degree (2005) in telecommunication engineering from Universitat Politècnica de València, València, Spain, and the Ph.D. degree (2010) in signal theory and communications, from the Universitat Politècnica de Catalunya (UPC), Barcelona, Spain.

In 2010, she joined the Department of Civil and Environmental Engineering, University of Melbourne, Australia, as a Research Fellow. From 2011 to 2015, she was a Research Scientist at UPC and Research Affiliate at Massachusetts Institute of Technology, Cambridge. In 2016, she joined the Institute of Marine Sciences, CSIC, as a Research Scientist. She is currently a “Ramón y Cajal” researcher at the Image Processing Laboratory, Universitat de València. Her research interests include microwave remote sensing, estimation of soil moisture and vegetation bio-geophysical parameters, and development of multi-sensor techniques for enhanced retrievals with focus on agriculture, forestry, wildfire prediction, extreme detection and climate studies.
\end{IEEEbiography} 


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/gustau.png}}]{Gustau Camps-Valls}
(M'04, SM'07, FM'18) Gustau Camps-Valls (IEEE Fellow'18, IEEE Distinguished lecturer, PhD in Physics) is currently a Full professor in Electrical Engineering and head of the Image and Signal Processing (ISP) group, http://isp.uv.es. He is interested in the development of machine learning algorithms for geosciences and remote sensing data analysis. He is an author of around 200 journal papers, more than 200 conference papers, 25 international book chapters, and editor of 5 books on kernel methods and deep learning. He holds a Hirsch's index h=63, entered the ISI list of Highly Cited Researchers in 2011, and Thomson Reuters ScienceWatch identified one of his papers on kernel-based analysis of hyperspectral images as a Fast Moving Front research. He received two European Research Council (ERC) grants: an ERC Consolidator grant on "Statistical learning for Earth observation data analysis" (2015) and an ERC Synergy grant on "Understanding and Modelling the Earth system with machine learning" (2019). In 2016 he was included in the prestigious IEEE Distinguished Lecturer program of the GRSS, and he's currently a fellow and coordinator of the European Lab for Learning & Intelligent Systems (ELLIS) program "Machine Learning for Earth Sciences".
\end{IEEEbiography} 


